Distributed-Memory Parallel Algorithms for Sparse Matrix and Sparse Tall-and-Skinny Matrix Multiplication

We consider a sparse matrix-matrix multiplication (SpGEMM) setting where one matrix is square and the other is tall and skinny. This special variant, called TS-SpGEMM, has important applications in multi-source breadth-first search, influence maximization, sparse graph embedding, and algebraic multigrid solvers. Unfortunately, popular distributed algorithms like sparse SUMMA deliver suboptimal performance for TS-SpGEMM. To address this limitation, we develop a novel distributed-memory algorithm tailored for TS-SpGEMM. Our approach employs customized 1D partitioning for all matrices involved and leverages sparsity-aware tiling for efficient data transfers. In addition, it minimizes communication overhead by incorporating both local and remote computations. On average, our TS-SpGEMM algorithm attains 5x performance gains over 2D and 3D SUMMA. Furthermore, we use our algorithm to implement multi-source breadth-first search and sparse graph embedding algorithms and demonstrate their scalability up to 512 Nodes (or 65,536 cores) on NERSC Perlmutter.

==> init_intro.tex <==
\section{Introduction}
Multiplication of two sparse matrices (SpGEMM) is a prevalent operation in scientific computing~\cite{bell2012exposing, devine2006parallel}, graph analytics~\cite{solomonik2017scaling, combblas2, Azad2018}, and machine learning~\cite{qin2020sigma}. 
Within these diverse applications, SpGEMM appears in three main variations: (a) $\mA\mA$, which involves squaring a sparse matrix $\mA\in \mathbb{R}^{n\times n}$, used in Markov clustering~\cite{Azad2018} and triangle counting~\cite{Azad2015}; 
(b) $\mA\mA\transpose$, which entails multiplying a matrix by its transpose, useful in calculating Jaccard similarity~\cite{besta2019communication}, performing sequence alignments~\cite{sc20pastis}, and conducting hypergraph partitioning~\cite{devine2006parallel}; and
 (c) $\mA\mB$, which involves multiplying two distinct sparse matrices, relevant in multi-source breadth-first search (BFS)~\cite{then2014more}, the initial phase of Algebraic Multigrid solvers~\cite{bell2012exposing}, influence maximization~\cite{minutoli2019fast}, and generating sparse graph embeddings. 
This paper focuses on a special instance of the final variant referred to as Tall-and-Skinny-SpGEMM (TS-SpGEMM), in which  $\mA\in \mathbb{R}^{n\times n}$ represents a square matrix and $\mB\in \mathbb{R}^{n\times d}$ denotes a tall and skinny matrix with $d\ll n$.

TS-SpGEMM plays a crucial role in both graph analytics and scientific computing applications. For instance, iterations of multi-source BFS traversals on a graph are equivalent to TS-SpGEMM operations, where $\mA$ is the adjacency matrix of the graph, and $\mB$ represents the BFS frontiers for all searches. Such multi-source BFS operations are central to calculations of influence maximization~\cite{minutoli2019fast} and closeness centrality~\cite{then2014more}, in which the sparsity of $\mB$ may vary significantly across iterations. Additionally, TS-SpGEMM is applicable in sparse graph embedding algorithms, where each row of $\mB$ corresponds to a $d$-dimensional sparse embedding of a vertex, and it is compatible \makis{I think compatible is not the best word choice here}
with graph neural networks (GNNs) that support sparse embeddings~\cite{rahman2022triple}. In the context of Algebraic Multigrid (AMG) methods, TS-SpGEMM is utilized during the setup phase, where $\mB$ is the restriction matrix created from a distance-2 maximal independent set computation~\cite{bell2012exposing}.

Despite its wide range of applications, TS-SpGEMM has not received focused attention in the literature (see Table~\ref{table:experimental-setting}). Current distributed-memory SpGEMM algorithms, such as Sparse SUMMA~\cite{Buluc2012, azad2016exploiting} in CombBLAS~\cite{combblas2} and 1-D partitioning-based algorithms in Trilinos~\cite{Heroux2005} and PETSc~\cite{Petsc2014}, perform well for standard scenarios but fall short in the TS-SpGEMM context, as demonstrated by our experiments. Our work aims to address this gap by introducing a scalable distributed-memory algorithm specifically designed for TS-SpGEMM.

Our TS-SpGEMM algorithm follows the principles of Gustavson's algorithm~\cite{Gustavson1978}, which constructs the output row-by-row. 
Since both input and output matrices are tall-and-skinny, 1-D partitioning is better suited for them.
For instance, in many cases, the number of columns in matrix $\mB$ could be fewer than the number of processes. 
However, a basic implementation of Gustavson's algorithm in distributed memory might necessitate fetching a substantial portion of $\mB$ into a process, potentially exceeding local memory capacity.
%1-D partitioning may lead to load imbalance depending on the sparsity of $\mA$.
We mitigate this issue by utilizing a 2-D virtual layout for matrix $\mA$ and conducting multiplications tile by tile, with each tile representing a submatrix of $\mA$ stored within a process. 
\makis{It is not very clear to me what the virtual layout means at this point and how it helps. Maybe we can say something along the lines of: during the execution of a tile only the memory footprint of B required by a specific tile of A needs to be stored in local memory reducing the concurrent memory footprint? Or is it obvious?}
By adjusting tile widths and heights, we can manage the granularity of computation and communication. 

We develop TS-SpGEMM with two modes for computations. 
In the {\em local compute} mode, $\mA$ and $\mC$ remain stationary, while data from $\mB$ is communicated to perform local multiplications.
Conversely, in the {\em remote compute} mode, $\mB$ and $\mC$ remain stationary, while data from $\mA$  is transferred to remote processes where multiplication is performed, and partial results are then returned back to their respective processes.
\makis{A detail: Partial C results are returned back, is C really stationary in this case?}
The choice of local and remote computations is determined for each tile based on its sparsity pattern.
\makis{Some intuition on how sparsity pattern affects this?}
By balancing local and remote computations, we can reduce communication costs for certain applications. 
As for local computations, we \makis{additionally} adaptively select between SPA or hash-based accumulator for local SpGEMM and merging of partial results.
These optimizations significantly enhance the performance of our TS-SpGEMM algorithm compared to existing distributed SpGEMM methods available in CombBLAS and PETSc.


We have developed \makis{implement} two graph algorithms: multi-source BFS and sparse graph embedding using TS-SpGEMM. 
In multi-source BFS, the output matrix from one iteration serves as the $\mB$ matrix in the subsequent iteration. Consequently, for scale-free graphs, the sparsity of $\mB$ fluctuates dramatically across BFS iterations. Regarding sparse embedding, we implemented a force-directed graph embedding algorithm~\cite{Force2Vec}, maintaining the embedding sparse without compromising its quality. In both scenarios, TS-SpGEMM offered substantial performance enhancements over other SpGEMM alternatives.

We summarize key contributions of this paper as follows:
\begin{itemize}[leftmargin=10pt]
\item {\bf New Algorithm}: We formulate TS-SpGEMM and develop a distributed-memory algorithm for this problem. 

\item {\bf Tiling}: TS-SpGEMM uses adaptive tiling to balance computational load. \makis{?}

\item {\bf Local/remote computations} TS-SpGEMM \makis{selectively} employs remote computations to reduce communication. 

\item {\bf TS-SpGEMM vs SpMM}: We demonstrate the scenario \makis{the conditions under} in which TS-SpGEMM outperforms sparse and tall-and-skinny dense matrix multiplication (SpMM).

\item {\bf TS-SpGEMM vs SUMMA}: We demonstrate the scenario \makis{the conditions under} in which TS-SpGEMM outperforms Sparse SUMMA.

\item {\bf Performance and Scalability}: For TS-SpGEMM (with $d=128$), our algorithm runs ** faster than alternative SpGEMM implementations in CombBLAS and PETSc. TS-SpGEMM scales well to 512 nodes (65,536 cores) on the Perlmutter supercomputer

\item {\bf Applications}: Multi-source BFS utilizing our TS-SpGEMM runs more than $10\times$ faster than SUMMA-enabled algorithms in CombBLAS.


\end{itemize}

\makis{Personal opinion is that I don't like a large list of contributions. I understand that we don't want to emphasize 1D partitioning since Trilinos and PETSc already do it. The Tiling contribution when mentioned in the intro paragraph appears to limit the memory footprint, nothing mentioned about balancing computation load. Also nothing mentioned about adaptive tiling (just tiling).} 



